Memory-Sample Tradeoffs for Linear Regression with Small Error

We consider the problem of performing linear regression over a stream of $d$-dimensional examples, and show that any algorithm that uses a subquadratic amount of memory exhibits a slower rate of convergence than can be achieved without memory constraints. Specifically, consider a sequence of labeled examples $(a_1,b_1), (a_2,b_2)\ldots,$ with $a_i$ drawn independently from a $d$-dimensional isotropic Gaussian, and where $b_i = \langle a_i, x\rangle + \eta_i,$ for a fixed $x \in \mathbb{R}^d$ with $\|x\|_2 = 1$ and with independent noise $\eta_i$ drawn uniformly from the interval $[-2^{-d/5},2^{-d/5}].$ We show that any algorithm with at most $d^2/4$ bits of memory requires at least $\Omega(d \log \log \frac{1}{\epsilon})$ samples to approximate $x$ to $\ell_2$ error $\epsilon$ with probability of success at least $2/3$, for $\epsilon$ sufficiently small as a function of $d$. In contrast, for such $\epsilon$, $x$ can be recovered to error $\epsilon$ with probability $1-o(1)$ with memory $O\left(d^2 \log(1/\epsilon)\right)$ using $d$ examples. This represents the first nontrivial lower bounds for regression with super-linear memory, and may open the door for strong memory/sample tradeoffs for continuous optimization.

==> overview_old.tex <==
\section{Setup and Proof Overview}

In this section, we provide an overview of our proof approach.  We begin by describing the notation and formalism we will use in analyzing the branching program representing a memory-bounded learning algorithm. 

\subsection*{Branching Program for Learning}

We model the learner by a branching program $B$. A branching program is a non-uniform and general model for space bounded computation. The branching program has $m$ layers, corresponding to $m$ time steps, with each layer having at most $w$ vertices, where $w$ denotes the \emph{width} of $B$. Each vertex of $B$ corresponds to a memory state, and a branching program with width $w$ corresponds to an algorithm with memory usage $\log_2 w$. A vertex with no outgoing edges is called a \emph{leaf}, and all vertices in the last layer are leaves (though there may be additional leaves). Each non-leaf vertex $v$ has an associated transition function $f_v: \mathbb{R}^d \times \mathbb{R} \rightarrow [w]$, representing the mapping from an example $(a,b)$ to a vertex in the next layer. Without loss of generality, we may assume that these transition functions are deterministic, as randomization can not improve the probability of success.\footnote{This can be easily seen by noting that any branching program with randomized transitions can be  converted to a deterministic one by iteratively derandomizing each vertex by replacing its randomized transition function with the deterministic one that select the transition that maximizes the probability of success (breaking ties arbitrarily), where the probability is taken over the randomization in the subsequent examples and whatever randomization remains in the transition functions corresponding to other vertices.}  To be consistent with the literature on branching programs, we will refer to this transition function as a series of `edges' indexed by the (infinite number of) potential examples $(a,b).$ Finally, each leaf vertex, $v$, of the branching program is labeled by a \emph{label}, $\tilde{x}(v)$, representing the output value that the corresponding algorithm would produce on the sequence of examples that led to vertex $v$. 

The success probability of $B$ for a specified accuracy parameter $\eps$ is the probability that $\norm{\td{x}-x}\le \eps$, where $\td{x}$ is the vector returned by $B$, and the probability is with respect to the randomness in the sequence of examples and choice of the true $x$.

\subsection*{Setup}

We consider branching programs whose goal is to learn some true $x\in \mathbb{R}^d$ with $\norm{x}=1$ to $\ell_2$ error $\eps$, in the setting where $x$ is drawn uniformly at random from the $d$ dimensional unit sphere. At every time step, a $d$-dimensional vector $a$ is sampled from $N(0,I_d)$, and the branching program is given $a$ and the (noisy) inner product $b=a^Tx+\eta$, where the noise $\eta$ is sampled from $U[-\delta,\delta]$ for $\delta=2^{-d/5}$.  The addition of this noise facilitates the analysis, and we could have equivalently assumed that the true inner product $a^Tx$ is discretized according to some exponentially small discretization error $\delta$. Note that as long as the goal is to estimate $x$ up to accuracy $\eps \ge 2^{-\gamma d}$ for a small constant $\gamma$, the small uniform noise or discretization does not create any information theoretic obstacles. %\sidford{If true formally, then we wouldn't need to assume right?} \valiant{I changed this last bit from ``is not an obstacle for any branching program for the problem."}

\subsection*{Proof Overview}

Our proof follows and builds on the recent analytic framework for showing time-space lower bounds developed in \citet{raz2017time}, and further extended in \citet{beame2018time} and \citet{garg2018extractor}. The analysis in our case is complicated by the fact that the gap in the sample complexity of first order and second order methods for regression is not very large, and depends on the desired error $\eps$. %\sidford{But why complicating? Is it because we need to be careful about the accuracy achieved? If so - would add that.}% In particular, first order methods which only use linear memory can indeed solve the problem with linear sample complexity, but the known upper bounds suggest that the number of samples required for first order methods depends on the desired error $\eps$. 
To capture this dependence of the sample complexity on $\eps$, we divide the branching program into multiple \emph{stages}, where a stage is a group of consecutive layers of the branching program. Each stage will intuitively correspond to the branching program reducing the $\ell_2$ error of the estimate of $x$ by a factor of two. We will argue that each of these stages cannot be too short if the algorithm has small memory. We now sketch the proof, describing the high-level framework of \citet{raz2017time} and how we adapt it to our setup.\\

As in \citet{raz2017time}, we define a truncated computation path $\cT$ which follows the computation path of the branching program $B$, but may stop before reaching a leaf vertex. The conditions under which $\cT$ stops before reaching a leaf vertex will depend on the stage of the branching program which $\cT$ is in. For any vertex $v$ in the branching program, let $\posterior$ be the posterior distribution of $x$ conditioned on being at $v$. The truncated path $\cT$ stops at any \emph{significant} vertex $s$ where $\norm{\significant}$ is larger than some threshold, where the threshold is chosen as a function of the  stage of the branching program being analyzed. Intuitively, if $\norm{\significant}$ is larger than a given threshold, then $\cT$ has more information about $x$ then we expect it to have at that stage. Most of the effort in \citet{raz2017time} and in our work goes into ensuring that the probability of any significant vertex is small enough  that the probability of $\cT$ stopping due to reaching a significant vertex is small.\\

We now sketch the argument for showing that the probability of reaching a significant vertex, $s,$ is small, for any stage $B_t$ of the branching program $B$. Let $L_i$ denote the set of all vertices in the $i$th layer of the $t$-th stage $B_t$. The following potential function tracks the progress which the $i$-th layer of $B_t$ has made towards a fixed significant vertex $s$ in $B_t$,
\begin{align*}
 \cZ_i = \sum_{v \in L_i}^{}\Pr(v)\cdot\ip{\posterior}{\significant}^{d/2} .
 \end{align*}
We claim that if  $\cZ_i$ is small and the significant vertex $s$ lies in the $i$-th layer of $B_t$, then the probability of $s$ must also be small. This follows because we define significant vertices as those for which $\norm{\significant}$ is large, and if $s$ is in the $i$th layer then $\cZ_i \ge \Pr(s)\cdot\norm{\significant}^{d}$. Hence our goal will be to show that $\cZ_i$ is small. Note that raising to the power of $d/2$ in our expression for $\cZ_i$ allows us to show that the probability of significant vertices is small enough that we can do a union bound over all vertices in the branching program, and $d/2$ is the largest power to which we can raise while keeping the contribution of the low probability events small. \\

We prove that $\cZ_i$ is small via an induction argument. We first show that $\cZ_0$ must be small, as the previous stage $B_{t-1}$ of the branching program could not have made too much progress. We next show that $\cZ_{i+1}$ cannot be much larger than $\cZ_i$. To show this, we introduce another potential which tracks how much progress any edge $e$ of the branching program has made towards $s$. Let $\edgeposterior$ be the posterior distribution of $x$ conditioned on the event of traversing edge $e$ in the branching program. Let $\Gamma_i$ denote the set of all edges from the $(i-1)$-th layer to the $i$-th layer of the $t$-th stage $B_t$ of the branching program, and let $p(e)$ be the p.d.f. of the distribution over edges evaluted at edge $e$. For any $i$, we define the potential,
\begin{align*}
\cZ_i' = \int\displaylimits_{\edge \in \Gamma_{i}}p(\edge)\cdot\ip{\edgeposterior}{\significant}^{ d/2}\; de.
\end{align*}
A straightforward convexity argument shows that $\cZ_{i+1}\le \cZ'_i$. Hence the main challenge is showing that $\cZ_i'$ cannot be much larger than $\cZ_i$. This is the part where our analysis differs significantly from \citet{raz2017time} (this is also where \citet{beame2018time} and \citet{garg2018extractor} differ the most from \citet{raz2017time}). In these previous works which concern learning over finite fields, the learning problem is viewed as a certain matrix, and properties of this matrix are used to show that $\cZ_i'$ cannot be much larger than $\cZ_i$. It is worth noting that in these settings, it is possible to argue that the example in the next time step looks almost random to the branching program if it does not have significant knowledge about the answer, and use this to show that the branching program cannot make too much progress when it gets an example. In our case though, first-order methods which require only linear memory \emph{can} learn $x$ up to non-negligible error with only linear sample complexity, hence the examples do not have as much randomness. Also, as we work over continuous spaces we lack the combinatorial properties that enables the analysis in the previous works to go through, and need to develop different tools.  \\

We now sketch our argument for showing that $\cZ_i'$ cannot be much larger than $\cZ_i$. For intuition, we first describe the argument as it would pertain to the branching program corresponding to the linear memory, first-order method for regression. At a high level, by the end of the $t$-th stage of this branching program, the algorithm has learned $x$ up to error roughly $\eps_t=1/2^t$, and the posterior $\posterior$ of a vertex $v$ in this stage roughly corresponds to a spherical Gaussian with standard deviation $\eps_t$ in every direction.  A target significant vertex, $s$, in the $t$-th stage will have posterior $\significant$ roughly corresponding to another spherical Gaussian, but with standard deviation $\eps_t/2$ in every direction.  This significant vertex represents a memory state that has learned significantly more than is expected of a vertex in this stage, and we will show that the probability of reaching such a vertex is small. As every example $(a,b)$ has some small uniform noise  $\eta\sim U[-\delta,\delta]$ added to $b$, if the branching program is initially at vertex $v$ and then gets the example $(a,b)$, the posterior $\posterior$ is updated by restricting it to the thin slice of the spherical Gaussian where $a^T x = [b-\delta,b+\delta]$. We need to argue that this slicing does not significantly increase the inner product with the posterior $\significant$ corresponding to the smaller, target Gaussian.  This holds, provided the target Gaussian does not have significantly higher probability mass in the slice to which we are restricting.  This is easy to analyze in this special setting where the posteriors are spherical Gaussians, by simply analyzing the projections of the two Gaussians along a random direction $a$.  In our actual proof, to bound the rate of progress via this argument, we cannot assume that the posteriors have such a nice form.  Nevertheless, we show a concentration result that guarantees that, for any distribution with sufficiently small $\ell_2$ norm, the projections can not behave too much worse than projections of spherical Gaussians with the corresponding $\ell_2$ norms.

%To Beyond this simple case where the posteriors are Gaussian, we can bound the rate of progress by showing concentration bounds for the projections of any distribution with small enough $\ell_2$ norm along a random direction $a$.

To sketch the argument more formally, we need to define some notation. We define $\td{f}$ as the point-wise product of the distributions $\posterior$ and $\significant$, with suitable normalization. Hence for any $x'$ on the $d$ dimensional unit sphere,
$$
\td{f}(x') = \frac{\posterior(x')\cdot \significant(x')}{\int\displaylimits_{z}\posterior(z)\cdot \significant(z)\; dz}\;.
$$
Let $I_{\delta}(b)$ be the interval $[b-\delta,b+\delta]$. For any distribution $f$ and fixed $a$, define   $G_{{f},a}(I_{\delta}(b)) = {\E_{x'\sim f}\Big[ \mathbf{1}(a^Tx'\in I_{\delta}(b)\Big]}$. Note that for a vertex $v$ with posterior distribution $\posterior$, $G_{\posterior,a}(I_{\delta}(b))$ is the probability mass on vectors $x'$ which are consistent with the example $(a,b)$, up to the noise level $\delta$. With some technical work, we can approximately relate $\ip{\posterior}{\significant}$ and $\ip{\edgeposterior}{\significant}$ for an edge $e$ labelled by $(a,b)$ as follows,
$$
\ip{\edgeposterior}{\significant} \approx \ip{\posterior}{\significant} \cdot \frac{G_{\td{f},a}(I_{\delta}(b))}{G_{\posterior,a}(I_{\delta}(b))}.
$$
Intuitively, the above relation  says that the progress that the truncated path $\cT$ makes towards some target distribution $\td{f}$ after receiving example $(a,b)$ depends on the ratio of the probability mass of $\td{f}$ which is consistent with $(a,b)$, and that of $\posterior$ which is consistent with $(a,b)$. Hence in order to bound $\E_e[\ip{\edgeposterior}{\significant}^{d/2}]$ in terms of $\ip{\posterior}{\significant}^{d/2}$, our goal will be to upper bound $$ \E_{a,b}\Big[\frac{G_{\td{f},a}(I_{\delta}(b))}{G_{\posterior,a}(I_{\delta}(b))}\Big]^{d/2}.$$
Note that as $b=a^Tx+\eta$ where $x\sim \posterior$, we can show that examples $(a,b)$ where $G_{\posterior,a}(I_{\delta}(b))$ is too small have small probability. Hence we can lower bound the denominator by making the truncated path $\cT$ stop if $G_{\posterior,a}(I_{\delta}(b))$ is too small, while still ensuring that the probability of $\cT$ stopping due to this reason is small.

It is more complicated to upper bound $\E_{a,b}[G_{\td{f},a}(I_{\delta}(b))^{d/2}]$. Note that $G_{\td{f},a}(I_{\delta}(b))$ is the probability mass of the distribution $\td{f}$ which lies in the interval $I_{\delta}(b)$ when $\td{f}$ is projected onto a random direction $a$. The linear projection of a high-dimensional distribution onto a random direction is a well-studied topic, and it is known that under mild conditions on $\td{f}$ such as bounded second moments, its projection onto a random direction is approximately Gaussian \citep{bobkov2003concentration,anttila2003central,von1997sudakov} or a mixture of Gaussians \citep{dasgupta2006concentration} with high probability. However, these results typically only give an additive $O(1/\sqrt{d})$ error guarantee for the difference between the probability mass of $\td{f}$ on any interval $I$ and that of an appropriate Gaussian on that interval (and this is tight given only second moment constraints). Note that in our case the intervals $I_{\delta}(b)$ have exponentially small width $\delta$, and we care about the multiplicative approximation error, hence these $O(1/\sqrt{d})$ additive error guarantees are not strong enough. We show that we can obtain stronger guarantees in our case by ensuring that $\norm{\td{f}}$ is small, which we guarantee by appropriate conditions on the truncated path $\cT$. With a bound on $\norm{\td{f}}$, we prove the following concentration result for projections of high-dimensional distributions onto a random direction---

\begin{lemma}\label{lem:upper_bnd_simple}
	Let $\td{f}$ be a distribution over the $d$ dimensional sphere, with $\norm{\td{f}}\le \frac{(100/\eps)^{d}}{C_d}$ for some $\eps\le 1$. For an absolute constant $C$ and fixed $b$, $$\E_a\Big[G_{\td{f},a}(I_{\delta}(b))^{d/2}\Big]\le (C\eps^{-20}\delta)^{d/2}.$$
\end{lemma}

Finally, note that the above bound is for a fixed $b$, but if the branching program knows $x$ to a small error then it also knows the inner product $b$ for any $a$ to a small error, hence the distribution of $b$ is itself highly dependent on $a$. To get around this, we prove a version of the above Lemma where $b$ is obtained by first sampling $x$ from $\posterior$ and then adding noise $\mu$ to $a^Tx$. These concentration bounds may be useful beyond this work, and it may be interesting to further develop our understanding of properties of the projection of high-dimensional distributions with small $\ell_2$ norm onto a random direction. 

%We show that with high probability $\ip{\edgeposterior}{\significant}$ cannot be much larger than $\ip{\posterior}{\significant}$. 

%In these previous works, the learning problem is viewed as a certain matrix, and properties of this matrix are used to show that  $\cZ_i'$ cannot be much larger than $\cZ_i$. 
